Defending Multimodal Fusion Models against Single-Source Adversaries

Beyond achieving high performance across many vision tasks, multimodal models are expected to be robust to single-source faults due to the availability of redundant information between modalities. In this paper, we investigate the robustness of multimodal neural networks against worst-case (i.e., adversarial) perturbations on a single modality. We first show that standard multimodal fusion models are vulnerable to single-source adversaries: an attack on any single modality can overcome the correct information from multiple unperturbed modalities and cause the model to fail. This surprising vulnerability holds across diverse multimodal tasks and necessitates a solution. Motivated by this finding, we propose an adversarially robust fusion strategy that trains the model to compare information coming from all the input sources, detect inconsistencies in the perturbed modality compared to the other modalities, and only allow information from the unperturbed modalities to pass through. Our approach significantly improves on state-of-the-art methods in single-source robustness, achieving gains of 7.8-25.2% on action recognition, 19.7-48.2% on object detection, and 1.6-6.7% on sentiment analysis, without degrading performance on unperturbed (i.e., clean) data.

==> benchmarks.tex <==
\section{Experiments}\label{sec:benchmarks}

\subsection{Multimodal Robustness Benchmarks}

\iffalse
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c|]
{@{}l@{}}Multimodal Robustness \\ Benchmarks\end{tabular} &
  Dataset &
  Task &
Evaluation Metrics &
  $k$ &
  Modality 1 &
  Modality 2 &
  Modality 3 \\ \hline \hline
Kim et al, \cite{kim2018robust, kim2018robusta} &
  KITTI &
  SUN-RGBD &
  Average Precision &
  2 &
  Visual frame &
  Depth Map &
  N/A \\ \hline
 Kim et al, \cite{kim2018robust, kim2018robusta} &
  KITTI &
  2D Object Detection &
  Average Precision &
  2 &
  Visual frame &
  Depth Map (Velodyne) &
  N/A \\ \hline
Kim \& Ghosh \cite{kim2019single} &
  KITTI &
  3D Object Detection &
  Average Precision &
  2 &
  Visual frame &
  Depth Map (Velodyne) &
  N/A \\ \hline \hline
Ours &
  EPIC-Kitchens &
  Action Recognition &
  Classification Accuracy &
  3 &
  Visual frames &
  Motion frames (Flow) &
  Audio \\ \hline
Ours &
  KITTI &
  2D Object Detection &
  Average Precision &
  3 &
  Visual frame &
  Depth Map (Velodyne) &
  Depth Map (Stereo) \\ \hline
Ours &
  CMU-MOSI &
  Sentiment Analysis &
  Classification Accuracy &
  3 &
  Visual frame &
  Audio &
  Text \\ \hline
\end{tabular}
\caption{Comparison of our multimodal robustness benchmark tasks against existing work.}
\label{table:benchmark_tasks}
\end{table*}

\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{|c|p{3.5cm}|c|p{5cm}|p{3cm}|}
    \hline
       Dataset  & Feature extractors&fusion  &Adversarial perturbation & Metric\\ \hline
       Epic-Kitchen  & Inception \cite{inception} &feed-forward network& 10-step PGD: $\epsilon = 8/256$ for video and motion, $\epsilon = 0.8$ for audio&top-1 and top-5 accuracy\\\hline
       KITTI   &Darknet \cite{darknet}&$1 \times 1$ convolutional layer&10-step PGD: $\epsilon = 8/256$ & average precision\\\hline
       MOSI   &Text: Transformer;Video: Facenet+LSTM; audio:MFCC+LSTM&feed-forward network&word replacement \cite{text_attack2} on 1 word per sentence; 10-step PGD: $\epsilon = 8/256$ for video, $\epsilon = 0.8$ for audio & binary and 7-class accuracy\\\hline
    \end{tabular}
    \caption{Feature extractors, fusion network $h$, and types of adversarial perturbations for Epic-Kitchen, KITTI, and MOSI. }
    \label{tab:exp_setup}
\end{table*}
\fi

\begin{table*}[]
\centering
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}} & \textbf{Tasks} & \textbf{Input Modalities} & \textbf{Model} & \textbf{Adversarial Perturbation} & \textbf{Evaluation Metrics} \\ \hline
\textbf{EPIC-Kitchens} \cite{} &
  \begin{tabular}[c]{@{}l@{}}Action \\ recognition\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Visual frames; \\ Motion frames (flow); \\ Audio (spectrogram)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Feature extractors: BNInception \cite{inception} (all);\\ Fusion: feed-forward network + temporal pooling;\\ Odd-one-out network: feed-forward network\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}10-step PGD \cite{}:\\ $\epsilon$ = 8/256 (vision) \\ $\epsilon$ = 8/256 (motion)\\ $\epsilon$ = 0.8 (audio)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Top-1, top-5 accuracy:\\ Verbs, nouns, actions\end{tabular} \\ \hline
\textbf{KITTI} \cite{}&
  \begin{tabular}[c]{@{}l@{}}2D object\\ detection\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Visual frame;\\ Depth map (Velodyne);\\ Depth map (stereo image)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Feature extractors: Darknet19 \cite{darknet} (all);\\ Fusion: 1 $\times$ 1 conv layer + YOLO \cite{};\\ Odd-one-out network: 1 $\times$ 1 conv net;\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}10-step PGD:\\ $\epsilon$ = 16/256 (all)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Average precision:\\ Cars (\textgreater{}0.7 IoU),\\ Pedestrians (\textgreater{}0.5 IoU), \\ Cyclists (\textgreater{}0.5 IoU)\end{tabular} \\ \hline
\textbf{MOSI} \cite{} &
  \begin{tabular}[c]{@{}l@{}}Sentiment\\ analysis\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Visual frame;\\ Audio (mel ceptron);\\ Text\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Feature extractors: FaceNet\cite{} +LSTM (vision), \\ MFCC+LSTM (audio), transformer \cite{} (text);\\ Fusion: feed-forward network\\ Odd-one-out network: feed-forward network\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}10-step PGD:\\ $\epsilon$ = 8/256 (vision)\\ $\epsilon$ = 0.8 (audio)\\ word replacement \cite{text_attack2}, \\ 1-word per sentence (text)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Binary accuracy\\ 7-class accuracy\end{tabular} \\ \hline
\end{tabular}
\end{table*}

To evaluate the robustness of multimodal models against single-source adversarial attacks, we propose three benchmark tasks. Existing benchmark tasks for studying single source corruptions in multimodal models have primarily focused on the object detection task with two modalities \cite{kim2019single, kim2018robust, kim2018robusta}. In contrast, our benchmarks involve three input modalities %with shared information (see Supplementary Materials for more details) 
and span a larger variety of tasks and data sources. %See Supplementary Materials for details about how we assess the level of redundancy between the modalities. %Below, we describe the datasets, modalities, and evaluation metrics for the proposed benchmarks.

%The robustness of multimodal models against single-source perturbations relies on the assumption that there is shared information between the data modalities. %If there is no redundant information between the modalities, then there is no reason to expect the modalities to compensate for each other in the case that there is a single-source error. 
%Therefore, we also provide a brief quantitative analysis and discussion of the level of data redundancy in each of our benchmarks in the Supplementary Materials.

%We designed these tasks with the following considerations: (1) each task should involve (at least) three input modalities with redundant information; (2) the tasks should encompass different types of modalities (\eg, visual, audio, text, LIDAR, \etc.) and objectives (\eg, classification, object detection) to ensure generality of the conclusions drawn about fusion methods; and (3) standardized downloads should be available for each of these tasks, to encourage consistency of the reported numbers in future work. 

\paragraph{Action recognition on EPIC-Kitchens.}
%
EPIC-Kitchens is the largest egocentric video dataset consisting of 39,596 video clips \cite{Damen2018EPICKITCHENS}. The objective is to predict the action taking place in the video, which is composed of one verb and one noun out of 126 and 331 classes respectively. %For training and evaluation, we propose to follow the splits proposed by Kazakos et al. \cite{}. Specifically, we split the dataset into a training set of 26074 videos and a validation set of 2398 videos. %\karren{we need to mention why we're not using the official test splits for evaluation (It's because (1) the test set labels are not released and we cannot generate the adversarial attacks, (2) we do so many evaluations (in terms of different fusions) that we can't submit all of those on the official server.)}
%
%\paragraph{Input Modalities.}
Three modalities are available from the original dataset: visual information (RGB frames), motion information (optical flow), and audio information. We chose this dataset over other video datasets because the audio in EPIC-Kitchens is highly-informative for the action recognition task \cite{}, whereas multimodal models trained on other datasets generally do not use the audio modality. %We use the publicly-available preprocessed visual and motion modalities from the dataset and preprocess the audio modality as described in Kazakos et al. \cite{}. 
For training and evaluation, we split the dataset into a training set of 26074 videos and a validation set of 2398 videos following the publicly available splits of Kazakos et al. \cite{Damen2018EPICKITCHENS}.

%\paragraph{Evaluation Metrics.}
%Models are evaluated on a held-out validation set of 2398 videos based on their top-1 and top-5 classification accuracy on the verb, noun, and action classes. We consider clean performance, as well as performance on data with single source perturbations against each modality defined in Equation \ref{eq:adv_perturb}.
%We evaluate the models based on their classification accuracy on clean data as well as worst-case single-source perturbed data. We consider Top-1 and Top-K classification accuracies of the verb, noun, and action (verb and noun must both be correct).

\iffalse
\paragraph{Analysis of Redundancy.}
The results of our assessment of the EPIC-Kitchens multimodal benchmark are shown in Supplementary Table \ref{table:epic-kitchens-task}. We observe a trend of diminishing returns on clean performance as we add more modalities to the model, which indicates that there is redundant information between the modalities.
%--- notice that the drop of performance is relatively small from the 3-modal models (row 8) to any of the 2-modal models (rows 5-7), especially for the verb and noun classification tasks. 
However, there is also a notable amount of complementary information between the modalities. For example, the visual modality contains more information for noun classification, and the motion modality contains more information for verb classification. Our findings are consistent with the observations in \cite{}.
\fi

\paragraph{Object Detection on KITTI.} 
KITTI \cite{KITTI_OD} is an autonomous driving dataset that contains stereo camera and LIDAR information for 2D object detection, where the objective is to draw bounding boxes around objects of interest from predefined classes, \ie, car, pedestrian, cyclist, etc. % For training and evaluation, we split the dataset into a training set of ? samples and a validation set of ? samples.
%
%\paragraph{Input Modalities.} 
Existing works use different combinations and processed versions of the available data modalities for object detection \cite{}. For the proposed benchmark, we consider the following three modalities based on common use in the literature: (1) RGB frames, which are used by the majority of detection methods, (2) LIDAR points projected to a sparse depth map \cite{} and (3) a depth map estimated from the stereo views \cite{}. 
%Details of the preprocessing of the LIDAR and stereo views can be found in the Supplementary Material. 
For training and evaluation, we split the dataset into a training set of 5983 samples and a validation set of 1497 samples.
%
%\paragraph{Evaluation Metric.}
%Models are evaluated based on their Average Precision (AP) on three object classes: cars, pedestrians, and cyclists. For the car class, true positives are bounding boxes with Intersection over Union (IoU) $ > 0.7$ with real bounding boxes. For the pedestrian and cyclist classes, true positives are bounding boxes with IoU $> 0.5$ with real bounding boxes. We consider clean performance, as well as performance on data with single source perturbations against each modality defined in Equation \ref{eq:adv_perturb}.

\iffalse
\paragraph{Analysis of Redundancy.} The results of our assessment of the KITTI multimodal benchmark are shown in Supplementary Table \ref{table:kitti-detection-task}. Here, we observe that each modality achieves high performance on the task individually. The improvement of clean performance when increasing the number of modalities from 1 to 3 is rather minimal. This demonstrates that the information between these three modalities is highly redundant, and there is little complementary information between the modalities.
\fi

\paragraph{Sentiment Analysis on CMU-MOSI.}
 Multimodal Opinion-level Sentiment Intensity Corpus (CMU-MOSI)\cite{zadeh2016mosi} is a multimodal dataset for sentiment analysis consisting of 93 video clips of movie reviews, each of which are divided into an average of 23.2 segments. %There are 89 distinct speakers with each video featuring only one speaker. 
%Each video is divided into multiple segments with an average of 23.2 segments per video. 
Each segment %has an average duration of 4.2 sec with around 12 words in it and 
is labeled with a continuous sentiment intensity between $[-3,3]$, where a positive and negative values indicates positive and negative sentiments respectively. The objective is to predict the sentiment on a binary scale (\ie, negative v. positive) or 7-class scale (\ie, rounding to the nearest integer). MOSI contains three modalities: text, video and audio. We split the dataset into a training set of 1759 segments and a test set of 440 segments.
%
%\paragraph{Input Modalities.}
.% The audio is preprocessed by extracting Mel-frequency cepstral coefficients (MFCCs) using Librosa \cite{mcfee2015librosa}. For video, a pretrained VGGFace2\cite{cao2018vggface2} model is used to extract the facial features from the frames. The text features are extracted using a GloVe model \cite{pennington2014glove} pretrained on Wikipedia.
%is given by the 300-dimensional  embedding pretrained on Wikipedia.
%
%\paragraph{Evaluation Metric.} Models are evaluated based on their binary classification accuracy (\ie, predicting which sentiments are positive and which are negative) as well as their classification accuracy of 7 sentiment classes \karren{How are these determined? By rounding to closest integer?}. We consider clean performance, as well as performance on data with single source perturbations against each modality defined in Equation \ref{eq:adv_perturb}.

\iffalse
\paragraph{Analysis of Data Redundancy.} The results of our assessment of CMU-MOSI benchmark are shown in Supplementary Table \ref{table:mosi-sentiment-task}. In this task, we also observe a high level of data redundancy between the input modalities, given by the trend of diminishing returns on clean performance as we add more modalities. Text is the modality that carries most information, and adding video improves the performance more than adding audio. %Comparing row 8 which uses all three modalities and row 7 which uses video and text, as well as comparing row 4 which uses video and audio with row 1 which uses only video, one can see that there exist strong redundancy between audio and video.
\fi

\iffalse
\textbf{MOSI sentiment analysis } \textbf{Manash}\\
\begin{itemize}
    \item \textit{Dataset and task description}\\
    Multimodal Opinion-level Sentiment Intensity Corpus (MOSI) \cite{zadeh2016mosi} is a multimodal dataset for sentiment analysis. It consists of 93 Youtube videos featuring movie reviews. There are 89 distinct speakers with each video featuring only one speaker. Each video is divided into multiple segments with an average of 23.2 segments per video. Each segment has an average duration of 4.2 sec with around 12 words in it and a sentiment intensity between [-3,3] where sentiments intensities below 0 are negative and above 0 are positive. The intensities are continuous values. \\ In this work, we perform for the following tasks:
    \begin{itemize}
    \item \textit{Binary Classification:} Predict sentiments where sentiment intensities above 0 are positive sentiments and below 0 are negative sentiments
    \item \textit{7 Class Classification:} Predict sentiments as highly negative, negative, weakly negative, neutral, weakly positive, positive and highly positive
    \item \textit{Regression:} Predict the continuous sentiment intensity value

    \end{itemize}
    \end{itemize}
\fi

==> supp_files/additional_tables.tex <==
\section{Additional Tables}

In the following, we provide additional results that were deferred from the main text due to space constraints. Supplementary Table \ref{table:supp-epic-kitchens} provides top-1 and top-5 accuracy of multimodal models on action recognition on EPIC-Kitchens and supplement the result of Table 2 in the main text. Supplementary Table \ref{table:kitti-robustness-results-1} shows average precision performance of multimodal models on easy/medium/hard object detection on the KITTI dataset and supplement the results of Table 3 in the main text. Supplementary Table \ref{table:end2endadversarial-results-mosi} shows end-to-end adversarial training results on MOSI -- the proposed method outperforms adversarial training on clean input for over 20\% with small sacrifice on robust accuracy.

\begin{table*}[]
\centering
\tiny
\begin{tabular}{|c|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{Clean} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Visual \\ Perturbation\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Motion \\ Perturbation\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Audio \\ Perturbation\end{tabular}} \\ \hline
\textbf{} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} \\ \hline
\textbf{Concat Fusion} &
  59.0 (86.1) &
  42.1 (66.5) &
  30.2 (60.8) &
  0.1 (25.0) &
  0.0 (7.3) &
  0.0   (4.0) &
  0.2   (24.6) &
  0.0 (5.1) &
  0.0 (2.7) &
  0.1 (21.2) &
  0.0 (6.8) &
  0.0 (3.5) \\ \hline
\textbf{Mean Fusion} &
  56.8 (85.9) &
  40.4 (66.1) &
  27.6 (59.7) &
  0.3 (58.1) &
  0.8 (15.8) &
  0.0 (11.8) &
  0.3 (64.2) &
  0.3 (14.3) &
  0.0 (12.0) &
  0.4 (48.0) &
  0.3 (16.9) &
  0.0 (12.0) \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{LEL+Robust \cite{kim2019single}} &
  61.2 (86.7) &
  \textbf{43.1 (68.9)} &
  30.5 (62.3) &
  22.3   (76.3) &
  11.6   (37.2) &
  6.6   (34.9) &
  25.4 (78.6) &
  24.6   (52.3) &
  12.0 (46.5) &
  20.4   (77.6) &
  17.7 (47.5) &
  8.0 (43.2) \\ \hline
\textbf{Gating+Robust \cite{kim2018robust,kim2018robusta}} &
  60.9 (87.6) &
  43.0 (68.7) &
  30.6 (62.8) &
  26.0 (77.9) &
  10.9 (42.0) &
  6.2 (39.0) &
  35.9 (83.6) &
  26.9 (58.3) &
  14.3 (52.5) &
  21.3 (79.9) &
  16.2 (51.4) &
  7.0 (47.2) \\ \hline
\textbf{Ours} &
  \textbf{61.5 (88.2)} &
  42.5 (68.4) &
  \textbf{31.4 (63.0)} &
  \textbf{48.0 (83.2)} &
  \textbf{24.2   (53.2)} &
  \textbf{16.8 (48.9)} &
  \textbf{48.5 (85.2)} &
  \textbf{35.6 (63.8)} &
  \textbf{22.1 (57.4)} &
  \textbf{46.5 (85.2)} &
  \textbf{33.3 (62.3)} &
  \textbf{22.1 (57.1)} \\ \hline
\end{tabular}
\vspace{0.1cm}
\caption{Top-1 (Top-5) classification accuracy results on EPIC-Kitchens dataset under clean data and single-source adversarial perturbations on each modality. Higher is better. See Table 2 in main paper and accompanying details in text for details.}
\label{table:supp-epic-kitchens}
\end{table*}


\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{|l|c|c|l|c|c|l|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{\textbf{Clean}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Visual (RGB)\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} \\ \hline
\textbf{Concat Fusion} &
  96.1 / 93.5 / 86.8 &
  85.7 / 81.5 / 77.0 &
  93.2 / 87.7 / 83.2 &
  15.6 / 14.3 / 14.8 &
  13.6 / 10.7 / 10.3 &
  13.8 / 12.3 / 12.9 \\ \hline
\textbf{Mean Fusion} &
  96.5 / 93.6 / 86.6 &
  84.3 / 77.7 / 73.4 &
  91.9 / 86.7 / 81.8 &
  13.2 / 12.6 / 13.1 &
  18.1 / 15.2 / 14.2 &
  11.9 / 10.5 / 10.2 \\ \hline
\textbf{LEL+Robust \cite{kim2019single}} &
  \multicolumn{1}{l|}{80.5 / 71.4 / 67.3} &
  \multicolumn{1}{l|}{69.0 / 64.2 / 61.3} &
  75.7 / 80.0 / 75.3 &
  \multicolumn{1}{l|}{3.71 / 3.95 / 4.62} &
  \multicolumn{1}{l|}{16.9 / 15.4 / 14.3} &
  16.4 / 13.9 / 13.2 \\ \hline
\textbf{Gating+Robust \cite{kim2018robust,kim2018robusta}} &
  \multicolumn{1}{l|}{90.6 / 89.4 / 82.8} &
  \multicolumn{1}{l|}{81.5 / 74.7 / 72.6} &
  92.9 / 84.6 / 81.8 &
  \multicolumn{1}{l|}{67.3 / 57.2 / 53.1} &
  \multicolumn{1}{l|}{62.0 / 54.2 / 50.7} &
  68.6 / 56.0 / 53.1 \\ \hline
\textbf{Ours} &
  \multicolumn{1}{l|}{95.6 / 90.6 / 83.9} &
  \multicolumn{1}{l|}{84.5 / 79.9 / 75.7} &
  90.4 / 85.4 / 80.6 &
  \multicolumn{1}{l|}{\textbf{89.6 / 85.1 / 78.9}} &
  \multicolumn{1}{l|}{\textbf{80.5 / 73.9 / 69.8}} &
  \textbf{87.9 / 82.3 / 77.6} \\ \hline
\end{tabular}

\begin{tabular}{|l|c|c|l|c|c|l|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Depth (Velo)\\ Perturbation\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Stereo Disparity\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} \\ \hline
\textbf{Concat Fusion} &
  3.43 / 1.58 / 1.59 &
  11.3 / 11.1 / 11.4 &
  8.72 / 8.82 / 8.22 &
  7.37 / 3.57 / 3.44 &
  8.08 / 4.64 / 4.36 &
  9.13 / 7.23 / 7.72 \\ \hline
\textbf{Mean Fusion} &
  6.77 / 3.16 / 2.90 &
  13.7 / 12.9 / 12.8 &
  10.1 / 7.88 / 8.07 &
  6.88 / 3.08 / 2.73 &
  9.17 / 8.03 / 8.81 &
  12.2 / 7.77 / 7.28 \\ \hline
\textbf{LEL+Robust \cite{kim2019single}} &
  \multicolumn{1}{l|}{7.30 / 6.83 / 6.73} &
  \multicolumn{1}{l|}{24.4 / 20.6 / 18.9} &
  28.8 / 24.8 / 24.7 &
  \multicolumn{1}{l|}{10.1 / 9.39 / 9.50} &
  \multicolumn{1}{l|}{26.0 / 24.2 / 21.8} &
  25.7 / 24.7 / 23.8 \\ \hline
\textbf{Gating+Robust \cite{kim2018robust,kim2018robusta}} &
  \multicolumn{1}{l|}{51.7 / 46.5 / 43.2} &
  \multicolumn{1}{l|}{53.5 / 45.7 / 42.1} &
  58.8 / 45.6 / 53.8 &
  \multicolumn{1}{l|}{43.9 / 41.6 / 38.8} &
  \multicolumn{1}{l|}{53.9 / 47.4 / 44.1} &
  60.0 / 48.8 / 46.8 \\ \hline
\textbf{Ours} &
  \multicolumn{1}{l|}{\textbf{92.8 / 87.8 / 79.4}} &
  \multicolumn{1}{l|}{\textbf{78.3 / 71.1 / 67.1}} &
  \textbf{88.9 / 85.8 / 81.1} &
  \multicolumn{1}{l|}{\textbf{92.8 / 89.8 / 83.1}} &
  \multicolumn{1}{l|}{\textbf{83.6 / 76.8 / 72.4}} &
  \textbf{88.1 / 84.7 / 79.9} \\ \hline
\end{tabular}
\caption{Evaluation of Average Precision for 2D object detection (easy/medium/hard difficulty) on the KITTI dataset under clean data and single-source adversarial perturbations on each modality. Higher is better. See Table 3 in main paper and accompanying details in text for details.}
\label{table:kitti-robustness-results-1}
\end{table*}


\begin{table*}[t]
\begin{center}
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{Fusion} & \multicolumn{2}{c|}{\textbf{Clean}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Audio\\ Perturbation\end{tabular}}}  & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Video\\ Perturbation\end{tabular}}}  & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Text\\ Perturbation\end{tabular}}}  \\
\hline
\textbf{} &
  \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
    \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
    \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
    \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
  \hline

\textbf{Adversarial training} &61.23 & 36.02&74.38 &42.13 &70.34 & 39.28&69.94 & 32.45 \\\hline
\textbf{Ours}    &\textbf{82.03} & \textbf{50.89}&73.18 & 42.06&69.94 & 38.20& 66.13 & 30.20\\\hline

\end{tabular}
\end{center}
\caption{Binary and seven-class classification results (\%) of end-to-end adversarial training and our method on MOSI. Higher is better. }
\label{table:end2endadversarial-results-mosi}
\end{table*}

==> supp_files/early_fusion.tex <==
\section{Early Fusion vs. Late Fusion Models}
In our preliminary experiments, we found that early fusion models are notably less robust than late fusion methods, which motivated us to focus on late fusion approaches in this work. Supplementary Table \ref{table:ucf101-early-late-fusion} shows our results comparing early and late fusion approaches on action recognition on the UCF-101 dataset. Here the input consists of 2-5 frames (which are treated as different views) and only one of the frames is adversarially perturbed while the others are clean An early fusion method that concatenates the frames over their spatial dimensions before passing them through a convolutional neural network is significantly less robust than a late fusion network that processes the frames individually and averages the output.

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
 &  & \multicolumn{4}{l|}{\textbf{Number of Input Frames}} \\ \hline
 & \textbf{Input Type} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \\ \hline
\multirow{2}{*}{\textbf{Early Fusion Model}} & Clean frames & 69.7/89.3 & 70.2/89.1 & 68.3/87.2 & 70.9/87.4 \\ \cline{2-6} 
 & Single-frame attack & 16.3/38.1 & 20.8/45.1 & 20.0/45.0 & 22.5/48.8 \\ \hline
\multirow{2}{*}{\textbf{Late Fusion Model}} & Clean frames & 72.4/89.0 & 73.0/90.0 & 74.0/89.6 & 73.5/90.5 \\ \cline{2-6} 
 & Single-frame attack & 46.9/76.4 & 62.0/83.5 & 66.7/85.8 & 67.0/87.4 \\ \hline
\end{tabular}
\caption{\textbf{Early fusion vs. late fusion robustness on UCF-101 action recognition.} The early fusion model is significantly less robust than the late fusion model under a single-frame perturbation. Top 1 / Top 5 classification accuracy is shown (higher is better). See text for details.}
\label{table:ucf101-early-late-fusion}
\end{table*}

We also evaluated the robustness of transformers that perform early fusion of video, audio, and text from the MOSI dataset, and found that they performed notably worse than late fusion models as shown in Supplementary Table \ref{table:MOSI-early-late-fusion}.


\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
 
 & \textbf{Audio} & \textbf{Video} & \textbf{Text} \\ \hline
\textbf{Early Fusion (transformer) Model} &  15.9 & 18.2 & 27.5  \\ \hline

\textbf{Late Fusion Model} &  56.92 & 51.23& 39.1 \\ \hline

\end{tabular}
\caption{\textbf{Early fusion vs. late fusion robustness on two-class MOSI sentiment analysis.} The early fusion model is significantly less robust than the late fusion model, especially under audio and video perturbation.}
\label{table:MOSI-early-late-fusion}
\end{table*}

One intuitive explanation for these results is the following: in early fusion models, there are multiple early interactions between attacked and clean modalities, so feature extraction becomes strongly influenced by the attacked input. In contrast, in late fusion models, feature extraction of the clean modalities is mostly shielded from the attack.

==> supp_files/implementation.tex <==

\section{Experimental Details}

\subsection{Model Architecture and Training}
\paragraph{Action Recognition on Epic-Kitchens.} We adapt the state-of-the-art temporal binding networks by Kazakos et al. \cite{kazakos2019epic}. This model extracts features from each of the three modalities using an Inception network with Batch Normalization \cite{inception}. The features from different modalities are ensembled using feed-forward networks with ReLU activation prior to temporal aggregation and prediction of a verb and noun class. We obtain a pretrained model on clean data following the data preprocessing, augmentation, and training steps of Kazakos et al. \cite{kazakos2019epic}. We then augment the model with the robust fusion strategy described in Section 3 of the main text and perform training according to Algorithm 1 using stochastic gradient descent with momentum $0.9$ and weight decay $5 \times 10^{-4}$ for $\sim$120 epochs with a learning rate of $1 \times 10^{-3}$.

\paragraph{Object Detection on KITTI.} We adapt a single-shot detector based on YOLOv2 \cite{redmon2017yolo9000} and YOLOv3 \cite{redmon2018yolov3} to the multimodal setting. The model extracts features from each of the three modalities using a Darknet19 network \cite{redmon2017yolo9000}. The features are fused using a $1 \times 1$ convolutional layer prior to predicting bounding boxes and confidences using a YOLO detector layer \cite{redmon2018yolov3}. We obtain the Velodyne depth map by projecting the Velodyne points to the 2D image plane using the calibration and projection matrices provided in the dataset \cite{KITTI_OD}, followed by dilation with a $5\times 5$ diamond kernel and bilateral smoothing. We obtain the stereo depth image using the pretrained PSMNet from \cite{wang2019pseudo}. All visual inputs are resized to $1280 \times 380$ for training and evaluation. During training, we augment the visual inputs by adding a random horizontal flip and a random shift that is at most one-fifth of the original width and height of the image, and we additionally augment the RGB image by randomly shifting the hue, exposure, and saturation. 
We obtain a pretrained multimodal model on unperturbed data in two steps: (i) we pretrain single-shot detectors for each modality using the same architecture, except for the fusion layer using stochastic gradient descent with momentum $0.9$ and weight decay $5\times 10^{-4}$ for $\sim$500 epochs with a learning rate of $1 \times 10^{-3}$, (ii) we train the fusion layer over the pretrained Darknet19 networks with the same optimization for $\sim$120 epochs. We then augment the model with the robust fusion strategy described in Section 3 of the main text and perform training according to Algorithm 1 using stochastic gradient descent (SGD) with momentum $0.9$, weight decay $5\times 10^{-4}$, and gradient clip of $20$ for $\sim$20 epochs with a learning rate of $1 \times 10^{-3}$.

\paragraph{Sentiment Analysis on CMU-MOSI.} For video input, we use VGGFace2 \cite{cao2018vggface2} followed by one layer of multi-head attention \cite{vaswani2017attention} and two layers of bi-directional LSTMs; for audio, we apply the same architecture on the Mel-frequency cepstral coefficients (MFCCs) of the audio signal instead of VGGFace2 outputs; for text, we apply the Transformer model \cite{vaswani2017attention} on a 300 dimensional pretrained GloVe embedding trained on Wikipedia from \cite{pennington2014glove}. We first train unimodal models using each of these three feature extractor followed by a fully-connected layer. We then augment the model with the robust fusion strategy described in Section 3 of the main text and perform training according to Algorithm 1 using stochastic gradient descent with momentum $0.9$, weight decay $5 \times 10^{-4}$, a learning rate of $1 \times 10^{-5}$, and trained for 40 epochs.

\subsection{Adversarial Perturbations}
The adversarial perturbations considered in our experiments are white box adaptive attack, \ie, attacks are generated with full knowledge of $f_{\text{robust}}$.

\paragraph{Action Recognition on EPIC-Kitchens.} We consider single-source $\ell_\infty$ attacks on each of three modalities: vision, motion, and audio. To generate the perturbations, we approximate the solution of Equation 1 of the main text using projected gradient descent (PGD) \cite{madry2017towards}, taking $\mathcal{L}$ to be the sum of the cross-entropy losses from the verb and noun classes. For vision and motion, we approximate the solution with 10-step PGD with $\epsilon = 8/256$. For the audio spectrogram, we approximate the solution with 10-step PGD with $\epsilon = 0.8$. %\karren{We observed empirically that the range of the audio inputs is approximately an order of magnitude smaller than that of vision and motion inputs.}

\paragraph{Object Detection on KITTI.} We consider single-source $\ell_\infty$ perturbations on each of three visual modalities. To generate the perturbations, we approximate the solution of Equation 1 in the main text using 10-step PGD with $\epsilon = 16/256$, taking $\mathcal{L}$ to be the YOLO loss \cite{redmon2018yolov3}. The loss consists of the cross-entropy losses of object and class confidences as well as the mean-squared localization errors summed over bounding box proposals.

\paragraph{Sentiment Analysis on CMU-MOSI.} We consider single-source attacks on each of three modalities: vision, audio, and text. The adversarial perturbations approximate the solution of Equation 1 in the main text, taking $\mathcal{L}$ to be the binary or 7-class cross entropy. For vision, we generate $\ell_\infty$ perturbations with 10-step PGD with $\epsilon = 8/256$. For audio, we generate the single-source $\ell_\infty$ perturbations with 10-step PGD with $\epsilon = 0.8$. For text, we adapted the word-replacement attack with priority based on word saliency \cite{text_attack2} with an attack budget of one word per sentence.

\subsection{Evaluation Metrics}
For each evaluation metric, we consider clean performance (\ie, performance on unperturbed data) as well as robust performance on data with single-source adversarial perturbations. For robust performance, we report the evaluation metric once for each attacked modality.

\paragraph{Action Recognition on EPIC-Kitchens.}
Models are evaluated based on their top-1 and top-5 classification accuracy on the verb, noun, and action classes. 

\paragraph{Object Detection on KITTI.}
We consider Average Precision (AP) on three object classes: cars, pedestrians, and cyclists. For the car class, true positives are bounding boxes with Intersection over Union (IoU) $ > 0.7$ with real boxes. For the pedestrian and cyclist classes, true positives are bounding boxes with IoU $> 0.5$ with real boxes.

\paragraph{Sentiment Analysis on CMU-MOSI.}
Models are evaluated based on their binary classification accuracy (\ie, predicting whether the sentiment is positive or negative) as well as their classification accuracy of 7 sentiment classes.

==> supp_files/kitti_clean.tex <==
\section{Clean performance of robust fusion strategy on KITTI}
Features that are trained on perturbed data are known to perform \textit{significantly} worse on unperturbed data \cite{madry2017towards}. In contrast, our approach is built on top of feature extractors pretrained on clean data and does not notably degrade clean performance. In the main text, we show across all three benchmarks that our performance on clean (unperturbed) data is comparable with fusion models with standard training (see the ``Clean'' column of the ``$\Delta$-Clean'' rows in Tables 2,3,4 of the main text). Clean performance seems slightly degraded on the KITTI dataset, but these differences are not significant when standard deviations are taken into account as shown in Supplementary Table \ref{table:kitti-clean-analysis}.

\begin{table}[]
\centering
\footnotesize
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Fusion}        & \multicolumn{3}{c|}{\textbf{Clean Performance}}         \\ \hline
\textbf{}              & \textbf{Car}   & \textbf{Pedestrian} & \textbf{Cyclist} \\ \hline
\textbf{Non-Robust Model} & 92.8 $\pm$ 1.3 & 81.0 $\pm$ 4.7      & 84.9 $\pm$ 4.7   \\ \hline
\textbf{Ours}          & 91.3 $\pm$ 2.7 & 80.8 $\pm$ 5.0      & 86.2 $\pm$ 4.5   \\ \hline
\end{tabular}
\caption{Clean performance of our robust model v. standard multimodal model, trained for the same number of epochs. The uncertainties shown are standard deviations computed over three splits of the validation data.}
\label{table:kitti-clean-analysis}
\end{table}
%

==> supp_files/oddoneout.tex <==





\section{Robust performance with different odd-one-out networks}
In Table 5 of the main text, we show that the odd-one-out network based on unaligned representations of different features is more effective at detecting the perturbed modality than a random baseline as well as an odd-one-out network based on aligned representations of the features. Supplementary Tables \ref{table:epic-kitchens-ooo}, \ref{table:kitti-ooo} and \ref{table:mosi-odd-one-out} show task performance of the models using different odd-one-out networks. Overall, we observe that task performance reflects the detection rates; when the model's odd-one-out network is more effective at detecting the perturbed modality, it is more successful at only allowing information from the unperturbed modalities to pass through the feature fusion step, resulting in better task performance under single-source perturbations. Specifically, we show that the model with the odd-one-out network based on unaligned representations of different features is more robust than the baselines that use a random odd-one-out network or an odd-one-out network based on aligned representations of the features.
%Here we conduct the same experiments as in Table \ref{table:detection_rate} but instead of detection rate, we report task performance (top1 accuracy for Epic-Kitchen, mAP for KITTI, and classification accuracy for MOSI.) for odd-one-out network with unaligned and aligned features, as well as random guessing which modality is under attack as baseline.


==> supp_files/oddoneout_results.tex <==
\begin{table*}[h!]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Odd-one-out network} &
  \multicolumn{3}{c|}{\textbf{Clean}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Visual\\ Perturbation\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Motion\\ Perturbation\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Audio\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} \\ \hline
\textbf{Random} &
  59.6 &
  \textbf{43.1} &
  30.1 &
  0.0 &
  0.0 &
  0.0 &
  0.0 &
  0.0 &
  0.0 &
  0.0 &
  0.0 &
  0.0 \\ \hline
\textbf{Unaligned features} &
  \textbf{61.5} &
  42.5 &
  \textbf{31.4} &
  \textbf{48.0} &
  \textbf{24.2} &
  \textbf{16.8} &
  \textbf{48.5} &
  \textbf{35.6} &
  \textbf{21.1} &
  \textbf{46.5} &
  \textbf{33.3} &
  \textbf{22.1} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Aligned features\\ (Logits)\end{tabular}} &
  \textbf{61.5} &
  38.0 &
  31.2 &
  38.7 &
  19.5 &
  13.1 &
  37.0 &
  29.1 &
  16.7 &
  31.1 &
  23.9 &
  13.8 \\ \hline
\end{tabular}
\caption{We show the top-1 classification accuracy of our fusion model with different odd-one-out networks on action recognition on the EPIC-Kitchens dataset under clean data and single-source adversarial perturbations on each modality. Higher is better.}
\label{table:epic-kitchens-ooo}
\end{table*}

\begin{table*}[h!]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline

\textbf{Odd-one-out network} &
  \multicolumn{3}{c|}{\textbf{Clean}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Visual (RGB)\\ Perturbation\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Depth (Velo)\\ Perturbation\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Stereo Disparity\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} \\ \hline
\textbf{Random} &
  90.1 &
  79.0 &
  84.3 &
  17.9 &
  7.6 &
  7.6 &
  1.8 &
  19.8 &
  28.1 &
  1.1 &
  18.4 &
  30.2 \\ \hline
\textbf{Unaligned features} &
  \textbf{90.6} &
  \textbf{79.9} &
  \textbf{85.4} &
  \textbf{85.1} &
  \textbf{73.9} &
  \textbf{82.3} &
  \textbf{87.8} &
  \textbf{71.1} &
  \textbf{85.8} &
  \textbf{89.8} &
  \textbf{76.8} &
  \textbf{84.7} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Aligned features\\ (Bounding Boxes)\end{tabular}} &
  90.2 &
  76.1 &
  83.3 &
  77.6 &
  66.5 &
  73.8 &
  83.1 &
  64.8 &
  68.3 &
  80.0 &
  65.1 &
  44.9 \\ \hline
\end{tabular}
\caption{We show the average precision (at medium difficulty) of our fusion model with different odd-one-out networks on object detection on the KITTI dataset under clean data and single-source adversarial perturbations on each modality. Higher is better.}
\label{table:kitti-ooo}
\end{table*}


\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{Odd-one-out network} & \multicolumn{2}{c|}{\textbf{Clean}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Audio\\ Perturbation\end{tabular}}}  & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Video\\ Perturbation\end{tabular}}}  & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Text\\ Perturbation\end{tabular}}}  \\
\hline
\textbf{} &
  \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
    \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
    \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
    \textbf{2-class} &
  \multicolumn{1}{c|}{\textbf{7-class}} &
  \hline
\textbf{Random} & 75.41 & 46.73 & 74.48 & 33.52.10 & 61.65 &31.46 & 62.98 & 25.01 \\ \hline

\textbf{Unaligned features}    &\textbf{82.03} & \textbf{50.89}&\textbf{73.18} & \textbf{42.06}&\textbf{69.94} & \textbf{38.20}& \textbf{66.13} & \textbf{30.20}\\\hline
%
\textbf{Aligned features} &80.13 & 48.26&71.95 & 39.74&66.47 & 35.43&60.74 & 26.57 \\\hline
\end{tabular}
\caption{We show the binary and 7-class accuracy of our fusion model with different odd-one-out networks on sentiment analysis on the CMU-MOSI dataset under clean data and single-source adversarial perturbations on each modality. Higher is better.}
\label{table:mosi-odd-one-out}
\end{table*}


==> supp_files/other_attacks.tex <==

\section{Other Types of Attacks}

In the main text of the paper, we showed across three benchmark tasks that standard multimodal models are not robust to single-source adversaries (\eg, end-to-end, untargeted white box attacks on the entire multimodal model) and subsequently proposed a defense strategy based on odd-one-out learning for robust feature fusion. Here, we show on the EPIC-Kitchens dataset that our results also hold for other types of attacks: transfer attacks, targeted attacks, and feature-level attacks \cite{xu2020towards}.

\paragraph{Transfer attacks.} We consider unimodal transfer attacks on the multimodal models by (1) training a unimodal classifier on top of pretrained feature extractors for each modality, (2) generating a white-box untargeted attack from this unimodal model, (3) applying the perturbed input to the multimodal model along with the two unperturbed inputs from the other modalities. Note that the perturbed input is generated without knowledge of the fusion model and without knowledge of the unperturbed inputs from other modalities. From the performance results of different models in Supplementary Table \ref{table:transfer-results-epic-kitchens}, we draw two conclusions. First, standard multimodal models based on concatenation fusion (``Concat Fusion'') or mean fusion (``Mean Fusion'') are also not robust to these transfer attacks, which are weaker than end-to-end white box attacks; in fact, the performance is close to zero, which is no better than a unimodal model defending against the same attack. In other words, an adversary can successfully attack a single modality of a multimodal model without knowledge of how features are fused between different modalities and without knowledge of the unperturbed inputs from other modalities. Second, our approach outperforms the standard models and existing state-of-the-art robust methods on these types of attacks (see ``$\Delta$-Clean'', ``$\Delta$-Robust''). We note, however, that all robust methods perform reasonably well against transfer attacks, as they are not adaptive attacks.

\paragraph{Feature-level attacks.} Feature level attacks, as proposed in \cite{xu2020towards}, are a good alternative way to assess the robustness of the fusion model, since here the attacker does not use the vulnerability of the feature extractors to generate the attack. To perform a feature-level attack, we perform a white-box attack on the feature representation for a particular modality after it has been extracted by a feature extractor $g_i$ and before it has been fused using $h$ (or $\tilde{h}$). We consider feature-level attacks with a maximum perturbation strength of $\epsilon=3$ for each modality. The performance results of different models are shown in Supplementary Table \ref{table:feature-results-epic-kitchens}. We note that standard multimodal models are also vulnerable to feature-level attacks; in fact, the performance is close to zero, which is no better than a unimodal model defending against the same attack. Additionally, our approach significantly outperforms the standard models and existing state-of-the-art robust methods on these types of attacks (see ``$\Delta$-Clean'', ``$\Delta$-Robust''). 


\paragraph{Targeted attacks.} To perform a targeted attack, we first randomly select a verb and noun class from the dataset and denote this target label as ${\hat{y}}$; we denote the predicted verb and noun for the input \textbf{x} as ${y}$. Subsequently, we generate a white-box adversarial attack against the model by optimizing Equation (1) of the main text, taking 
$$\mathcal{L}(f(x_i + \delta, \textbf{x}_{-i}), {\hat{y}}) = -\log \mathbb{P}_f(y = \hat{y}; x_i + \delta, \textbf{x}_{-i}).$$ 
The performance results of different models are shown in Supplementary Table \ref{table:targeted-results-epic-kitchens}. Importantly, our approach also outperforms the standard models and existing state-of-the-art robust methods on these types of attacks (see ``$\Delta$-Clean'', ``$\Delta$-Robust''). Note that the standard models appear to perform better than zero here; however, this is mainly because there is a chance of sampling targeted verb and noun classes that are the same as the real labels.



==> supp_files/other_attacks_results.tex <==

\begin{table*}[hbt!]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{\textbf{Clean}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Visual} \\ \textbf{Perturbation}\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Motion} \\ \textbf{Perturbation}\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Audio} \\ \textbf{Perturbation}\end{tabular}} \\ \hline
\textbf{} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} \\ \hline
 \textbf{Oracle (Upper Bound)} &
  - &
  - &
  - &
  55.8 &
  31.4 &
  21.9 &
  50.0 &
  37.2 &
  23.8 &  
  53.9 &
  39.2 &
  25.6
 \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{Concat Fusion} &
  59.0 &
  42.1 &
  30.2 &
  1.3 &
  0.8 &
  0.3 &
  0.5 &
  1.7 &
  0.1 &
  1.5 &
  2.1 &
  0.4 \\ \hline
\textbf{Mean Fusion} &
  56.8 &
  40.4 &
  27.6 &
  2.3 &
  0.8 &
  0.4 &
  0.4 &
  1.3 &
  0.1 &
  1.9 &
  2.5 &
  0.5 \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{LEL+Robust \cite{kim2019single}} &
  61.2 &
  \textbf{43.1} &
  30.5 &
  54.5 &
  30.4  &
  21.1 &
  51.4 &
  36.6 &
  22.7 &
  51.5  &
  37.3 &
  23.9 \\ \hline
\textbf{Gating+Robust \cite{kim2018robust, kim2018robusta}} &
  60.9 &
  43.0 &
  30.6 &
  56.9 &
  32.5 &
  22.7 &
  52.0 &
  \textbf{39.9} &
  25.2 &
  55.6 &
  39.4 &
  26.3 \\ \hline
\textbf{Ours} &
  \textbf{61.5 } &
  42.5 &
  \textbf{31.4} &
  \textbf{58.0} &
  \textbf{33.9} &
  \textbf{24.5} &
  \textbf{53.2} &
  39.2 &
  \textbf{25.6} &
  \textbf{56.6} &
  \textbf{39.5} &
  \textbf{27.1} \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
  %
  \textbf{$\Delta$-Clean} &
  \textbf{2.5} &
  \textbf{0.3} &
  \textbf{1.2} &
  \textbf{55.7} &
  \textbf{33.1} &
  \textbf{24.1} &
  \textbf{52.7} &
  \textbf{37.5} &
  \textbf{25.5} &
  \textbf{54.7} &
  \textbf{37.0} &
  \textbf{26.6} \\ \hline
  \textbf{$\Delta$-Robust} &
  \textbf{0.3 } &
  -0.6 &
  \textbf{0.8} &
  \textbf{1.1} &
  \textbf{1.4} &
  \textbf{1.8} &
  \textbf{1.2} &
  -0.7 &
  \textbf{0.4} &
  \textbf{1.0} &
  \textbf{0.1} &
  \textbf{0.8} \\ \hline
\end{tabular}
\vspace{0.1cm}
\caption{\textbf{Unimodal transfer attack.} Top-1 classification accuracy results on EPIC-Kitchens dataset under clean data and single-source adversarial perturbations on each modality, where the adversarial perturbations are generated and transferred from unimodal models. Higher is better. 
}
\label{table:transfer-results-epic-kitchens}
\end{table*}

\begin{table*}[hbt!]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{\textbf{Clean}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Visual} \\ \textbf{Perturbation}\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Motion} \\ \textbf{Perturbation}\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Audio} \\ \textbf{Perturbation}\end{tabular}} \\ \hline
\textbf{} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} \\ \hline
 \textbf{Oracle (Upper Bound)} &
  - &
  - &
  - &
  55.8 &
  31.4 &
  21.9 &
  50.0 &
  37.2 &
  23.8 &  
  53.9 &
  39.2 &
  25.6
 \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{Concat Fusion} &
  59.0 &
  42.1 &
  30.2 &
  0.0 &
  0.0 &
  0.0 &
  0.3 &
  0.1 &
  0.0 &
  0.0 &
  0.0 &
  0.0 \\ \hline
\textbf{Mean Fusion} &
  56.8 &
  40.4 &
  27.6 &
  0.1 &
  0.0 &
  0.0 &
  0.2 &
  0.0 &
  0.0 &
  0.0 &
  0.0 &
  0.0 \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{LEL+Robust \cite{kim2019single}} &
  55.8 &
  36.7 &
  23.9 &
  9.4 &
  7.2  &
  3.1 &
  11.3 &
  17.8 &
  5.1 &
  6.2 &
  12.3 &
  3.1 \\ \hline
\textbf{Gating+Robust \cite{kim2018robust, kim2018robusta}} &
  57.1 &
  39.1 &
  26.6 &
  18.8 &
  12.6 &
  6.7 &
  32.3 &
  25.7 &
  14.2 &
  16.3 &
  13.0 &
  7.6 \\ \hline
\textbf{Ours} &
  \textbf{60.2} &
  \textbf{42.5} &
  \textbf{31.0} &
  \textbf{53.6} &
  \textbf{29.7} &
  \textbf{20.8} &
  \textbf{48.7} &
  \textbf{35.6} &
  \textbf{22.7} &
  \textbf{50.7} &
  \textbf{36.4} &
  \textbf{23.5} \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
  %
  \textbf{$\Delta$-Clean} &
  \textbf{1.2} &
  \textbf{0.4} &
  \textbf{0.8} &
  \textbf{53.5} &
  \textbf{29.7} &
  \textbf{20.8} &
  \textbf{48.4} &
  \textbf{35.5} &
  \textbf{22.7} &
  \textbf{50.7} &
  \textbf{36.4} &
  \textbf{23.5} \\ \hline
  \textbf{$\Delta$-Robust} &
  \textbf{3.1} &
  \textbf{3.4} &
  \textbf{4.4} &
  \textbf{34.8} &
  \textbf{17.1} &
  \textbf{14.1} &
  \textbf{16.4} &
  \textbf{9.9} &
  \textbf{8.5} &
  \texetbf{34.4} &
  \textbf{23.4} &
  \textbf{15.9} \\ \hline
\end{tabular}
\vspace{0.1cm}
\caption{\textbf{Feature-level attack.} Top-1 classification accuracy results on EPIC-Kitchens dataset under clean data and single-source adversarial perturbations on each modality, where the adversarial perturbations are generated at the feature-level, rather than the input level, as proposed in \cite{xu2020towards}. Higher is better. 
}
\label{table:feature-results-epic-kitchens}
\end{table*}

\begin{table*}[hbt!]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{\textbf{Clean}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Visual} \\ \textbf{Perturbation}\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Motion} \\ \textbf{Perturbation}\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Audio} \\ \textbf{Perturbation}\end{tabular}} \\ \hline
\textbf{} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} \\ \hline
 \textbf{Oracle (Upper Bound)} &
  - &
  - &
  - &
  55.8 &
  31.4 &
  21.9 &
  50.0 &
  37.2 &
  23.8 &  
  53.9 &
  39.2 &
  25.6
 \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{Concat Fusion} &
  59.0 &
  42.1 &
  30.2 &
  15.9 &
  5.5 &
  2.0 &
  18.8 &
  8.4 &
  2.6 &
  15.9 &
  8.1 &
  2.6 \\ \hline
\textbf{Mean Fusion} &
  56.8 &
  40.4 &
  27.6 &
  23.9 &
  12.4 &
  5.3 &
  25.3 &
  14.3 &
  5.3 &
  22.6 &
  13.4 &
  4.0 \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{LEL+Robust \cite{kim2019single}} &
  \textbf{62.3} &
  42.3 &
  31.0 &
  31.6 &
  23.1  &
  6.7 &
  38.5 &
  32.2 &
  14.8 &
  31.5 &
  28.7 &
  9.6 \\ \hline
\textbf{Gating+Robust \cite{kim2018robust, kim2018robusta}} &
  61.9 &
  \textbf{44.7} &
  \textbf{31.9} &
  35.7 &
  25.9 &
  9.3 &
  45.9 &
  36.2 &
  19.5 &
  38.2  &
  28.8 &
  11.8 \\ \hline
\textbf{Ours} &
  60.8 &
  43.5 &
  31.3 &
  \textbf{45.1} &
  \textbf{32.1} &
  \textbf{17.5} &
  \textbf{51.5} &
  \textbf{38.0} &
  \textbf{24.5} &
  \textbf{56.6} &
  \textbf{40.0} &
  \textbf{27.7} \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
  %
  \textbf{$\Delta$-Clean} &
  \textbf{1.8} &
   \textbf{1.4} &
   \textbf{1.1} &
   \textbf{21.2} &
   \textbf{19.7} &
   \textbf{12.2} &
   \textbf{26.2} &
   \textbf{23.7} &
   \textbf{19.2} &
   \textbf{34.0} &
   \textbf{26.6} &
   \textbf{23.7} \\ \hline
  \textbf{$\Delta$-Robust} &
   -1.5 &
   -1.2 &
   -0.6 &
   \textbf{9.4} &
   \textbf{6.2} &
   \textbf{8.2} &
   \textbf{5.6} &
   \textbf{1.8} &
   \textbf{5.0} &
   \textbf{18.4} &
   \textbf{11.2} &
   \textbf{15.9} \\ \hline
\end{tabular}
\vspace{0.1cm}
\caption{\textbf{Untargeted attack.} Top-1 classification accuracy results on EPIC-Kitchens dataset under clean data and single-source adversarial perturbations on each modality, where the adversarial perturbations are generated to target the verb and noun class of a randomly sampled clip from the dataset, rather than the real verb and noun class. Higher is better. 
}
\label{table:targeted-results-epic-kitchens}
\end{table*}


==> supp_files/results_dump.tex <==
\begin{table*}[t]
\centering
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Model & \multicolumn{3}{c|}{Perturbed Vision} & Model & \multicolumn{3}{c|}{Perturbed Motion} & Model & \multicolumn{3}{c|}{Perturbed Audio} \\ \hline
%
 & Clean & Adv & Adv-F & & Clean & Adv & Adv-F & & Clean & Adv & Adv-F \\ \hline
%
Vision (LB) & 18.7 (54.2) & 0.0 (0.8) & 0.0 (0.0) &  Motion (LB) & 19.0 (48.4) & 0.0 (0.5) & 0.0 (0.0) &   Audio (LB) & 12.1 (35.9) & 0.0 (0.1) & 0.0 (0.0) \\ \hline
%
Concat Fusion & 30.2 (60.8) & 0.1 (8.9) & 0.0 (2.8) &   Concat Fusion & 30.2 (60.8) & 0.1 (7.5) & 0.0 (1.8) &   Concat Fusion & 30.2 (60.8) & 0.2 (8.1) & 0.0 (1.5) \\ \hline
%
Mean Fusion & 27.9 (59.7) & 0.0 (20.2) & 0.0 (8.8) &   Mean Fusion & 27.9 (59.7) & 0.0 (10.7) & 0.0 (10.7) &   Mean Fusion & 27.9 (59.7) & 0.0 (4.6) & 0.0 (4.6) \\ \hline
%
Motion+Audio (UB) & 21.9 (52.2) & 21.9 (52.2) & 21.9 (52.2) &   Vision+Audio (UB) & 23.8 (55.9) & 23.8 (55.9) & 23.8 (55.9) &   Motion+Audio (UB) & 25.6 (58.2) & 25.6 (58.2) & 25.6 (58.2) \\ \hline
\end{tabular}
\vspace{0.1cm}
\caption{Top-1 classification accuracy results on EPIC-Kitchens dataset. Higher is better. Standard multimodal fusion layers (mean, concat) are evaluated under single-source adversarial perturbations. LB = lower bound given by a unimodal model. UB = upper bound given by a multimodal model that excludes the perturbed modality.  Although there are three input modalities, perturbations (Adv, Adv-F) on a single modality are surprisingly effective, even when the adversary does not have access to the fusion layer weights (Adv-F). \karren{Full tables with results of top-5 classification accuracy, feature-level attack, noisy and mismatch corruptions are relegated to Supplementary Material but should be mentioned in the text.}}
\label{table:standard-fusion-epic-kitchens}
\end{table*}








\begin{table*}[t]
\centering
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Car detection & \multicolumn{3}{c|}{Perturbed RGB} & Model & \multicolumn{3}{c|}{Perturbed LIDAR} & Model & \multicolumn{3}{c|}{Perturbed Stereo} \\ \hline
%
 & Clean & Adv & Adv-F & & Clean & Adv & Adv-F & & Clean & Adv & Adv-F \\ \hline
%
RGB (LB) & 18.7 (54.2) & 0.0 (0.8) & 0.0 (0.0) &  %
LIDAR (LB) & 19.0 (48.4) & 0.0 (0.5) & 0.0 (0.0) & %
Stereo (LB) & 12.1 (35.9) & 0.0 (0.1) & 0.0 (0.0) \\ \hline
%
Concat Fusion & 30.2 (60.8) & 0.1 (8.9) & 0.0 (2.8) &  %
Concat Fusion & 30.2 (60.8) & 0.1 (7.5) & 0.0 (1.8) & %
Concat Fusion & 30.2 (60.8) & 0.2 (8.1) & 0.0 (1.5) \\ \hline
%
Mean Fusion & 27.9 (59.7) & 0.0 (20.2) & 0.0 (8.8) & %
Mean Fusion & 27.9 (59.7) & 0.0 (10.7) & 0.0 (10.7) &  %
Mean Fusion & 27.9 (59.7) & 0.0 (4.6) & 0.0 (4.6) \\ \hline
%
LIDAR+Stereo (UB) & 21.9 (52.2) & 21.9 (52.2) & 21.9 (52.2) & %
RGB+Stereo (UB) & 23.8 (55.9) & 23.8 (55.9) & 23.8 (55.9) &  %
RGB+LIDAR (UB) & 25.6 (58.2) & 25.6 (58.2) & 25.6 (58.2) \\ \hline \hline
%
%
Pedestrian detection & \multicolumn{3}{c|}{Perturbed RGB} & Model & \multicolumn{3}{c|}{Perturbed LIDAR} & Model & \multicolumn{3}{c|}{Perturbed Stereo} \\ \hline
%
 & Clean & Adv & Adv-F & & Clean & Adv & Adv-F & & Clean & Adv & Adv-F \\ \hline
%
RGB (LB) & 18.7 (54.2) & 0.0 (0.8) & 0.0 (0.0) &  %
LIDAR (LB) & 19.0 (48.4) & 0.0 (0.5) & 0.0 (0.0) & %
Stereo (LB) & 12.1 (35.9) & 0.0 (0.1) & 0.0 (0.0) \\ \hline
%
Concat Fusion & 30.2 (60.8) & 0.1 (8.9) & 0.0 (2.8) &  %
Concat Fusion & 30.2 (60.8) & 0.1 (7.5) & 0.0 (1.8) & %
Concat Fusion & 30.2 (60.8) & 0.2 (8.1) & 0.0 (1.5) \\ \hline
%
Mean Fusion & 27.9 (59.7) & 0.0 (20.2) & 0.0 (8.8) & %
Mean Fusion & 27.9 (59.7) & 0.0 (10.7) & 0.0 (10.7) &  %
Mean Fusion & 27.9 (59.7) & 0.0 (4.6) & 0.0 (4.6) \\ \hline
%
LIDAR+Stereo (UB) & 21.9 (52.2) & 21.9 (52.2) & 21.9 (52.2) & %
RGB+Stereo (UB) & 23.8 (55.9) & 23.8 (55.9) & 23.8 (55.9) &  %
RGB+LIDAR (UB) & 25.6 (58.2) & 25.6 (58.2) & 25.6 (58.2) \\ \hline \hline
%
%
%
Cyclist detection & \multicolumn{3}{c|}{Perturbed RGB} & Model & \multicolumn{3}{c|}{Perturbed LIDAR} & Model & \multicolumn{3}{c|}{Perturbed Stereo} \\ \hline
%
 & Clean & Adv & Adv-F & & Clean & Adv & Adv-F & & Clean & Adv & Adv-F \\ \hline
%
RGB (LB) & 18.7 (54.2) & 0.0 (0.8) & 0.0 (0.0) &  %
LIDAR (LB) & 19.0 (48.4) & 0.0 (0.5) & 0.0 (0.0) & %
Stereo (LB) & 12.1 (35.9) & 0.0 (0.1) & 0.0 (0.0) \\ \hline
%
Concat Fusion & 30.2 (60.8) & 0.1 (8.9) & 0.0 (2.8) &  %
Concat Fusion & 30.2 (60.8) & 0.1 (7.5) & 0.0 (1.8) & %
Concat Fusion & 30.2 (60.8) & 0.2 (8.1) & 0.0 (1.5) \\ \hline
%
Mean Fusion & 27.9 (59.7) & 0.0 (20.2) & 0.0 (8.8) & %
Mean Fusion & 27.9 (59.7) & 0.0 (10.7) & 0.0 (10.7) &  %
Mean Fusion & 27.9 (59.7) & 0.0 (4.6) & 0.0 (4.6) \\ \hline
%
LIDAR+Stereo (UB) & 21.9 (52.2) & 21.9 (52.2) & 21.9 (52.2) & %
RGB+Stereo (UB) & 23.8 (55.9) & 23.8 (55.9) & 23.8 (55.9) &  %
RGB+LIDAR (UB) & 25.6 (58.2) & 25.6 (58.2) & 25.6 (58.2) \\ \hline \hline


\end{tabular}
\vspace{0.1cm}
\caption{Average precision results on the EPIC-Kitchens dataset for car, pedestrian, and cyclist object classes. Higher is better. Standard multimodal fusion layers (mean, concat) are evaluated under single-source adversarial perturbations. Evaluation on Easy/Medium/Hard examples, following guidelines of KITTI evaluation server. LB = lower bound given by a unimodal model. UB = upper bound given by a multimodal model that excludes the perturbed modality. Although there are three input modalities, perturbations (Adv, Adv-F) on a single modality are surprisingly effective, even when the adversary does not have access to the fusion layer weights (Adv-F).}
\label{table:standard-fusion-kitti}
\end{table*}


\begin{table*}[]
\centering
\tiny
\begin{tabular}{|c|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{Clean} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Visual \\ Perturbation\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Motion \\ Perturbation\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Audio \\ Perturbation\end{tabular}} \\ \hline
\textbf{} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} &
  \multicolumn{1}{c|}{\textbf{Verb}} &
  \multicolumn{1}{c|}{\textbf{Noun}} &
  \multicolumn{1}{c|}{\textbf{Action}} \\ \hline
\textbf{Concat Fusion} &
  59.0 (86.1) &
  42.1 (66.5) &
  30.2 (60.8) &
  0.1 (25.0) &
  0.0 (7.3) &
  0.0   (4.0) &
  0.2   (24.6) &
  0.0 (5.1) &
  0.0 (2.7) &
  0.1 (21.2) &
  0.0 (6.8) &
  0.0 (3.5) \\ \hline
\textbf{Mean Fusion} &
  56.8 (85.9) &
  40.4 (66.1) &
  27.6 (59.7) &
  0.3 (58.1) &
  0.8 (15.8) &
  0.0 (11.8) &
  0.3 (64.2) &
  0.3 (14.3) &
  0.0 (12.0) &
  0.4 (48.0) &
  0.3 (16.9) &
  0.0 (12.0) \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|}
\textbf{Concat Fusion} &
  61.2 (86.7) &
  \textbf{43.1 (68.9)} &
  30.5 (62.3) &
  22.3   (76.3) &
  11.6   (37.2) &
  6.6   (34.9) &
  25.4 (78.6) &
  24.6   (52.3) &
  12.0 (46.5) &
  20.4   (77.6) &
  17.7 (47.5) &
  8.0 (43.2) \\ \hline
\textbf{Feature Gating} &
  60.9 (87.6) &
  43.0 (68.7) &
  30.6 (62.8) &
  26.0 (77.9) &
  10.9 (42.0) &
  6.2 (39.0) &
  35.9 (83.6) &
  26.9 (58.3) &
  14.3 (52.5) &
  21.3 (79.9) &
  16.2 (51.4) &
  7.0 (47.2) \\ \hline
\textbf{Ours} &
  \textbf{61.5 (88.2)} &
  42.5 (68.4) &
  \textbf{31.4 (63.0)} &
  \textbf{48.0 (83.2)} &
  \textbf{24.2   (53.2)} &
  \textbf{16.8 (48.9)} &
  \textbf{48.5 (85.2)} &
  \textbf{35.6 (63.8)} &
  \textbf{22.1 (57.4)} &
  \textbf{46.5 (85.2)} &
  \textbf{33.3 (62.3)} &
  \textbf{22.1 (57.1)} \\ \hline
\end{tabular}
\vspace{0.1cm}
\caption{Top-1 (Top-5) classification accuracy results on EPIC-Kitchens dataset under clean data (columns 2-4) and single-source adversarial perturbations (columns 5-12) on each modality. Higher is better. \textbf{Note 1}: Adversarial training of all fusion layers (rows 5-7) improves robustness to single-source  without negatively impacting clean accuracy compared to clean training (rows 3-4); in fact, clean accuracy is slightly improved. \textbf{Note 2}: Our fusion layer (row 7) significantly improves single-source adversarial robustness over existing fusion layers (rows 5-6). }
\label{table:standard-fusion-kitti}
\end{table*}

\begin{table*}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Model & Clean input & Audio attack & Video attack  & Text attack \\
\hline\hline
Naiive concat. fusion & 78.09 / 46.14& 53.21 / 20.51 & 43.15 / 18.17 & 33.14 / 8.23 \\
Naiive mean fusion & 81.82 / 46.69 & 56.92 / 21.38 & 51.23 / 19.75 & 39.50 / 9.97\\
Context-gated concat. fusion &78.82 / 46.37&69.31 / 38.26&64.23 / 31.88&59.39 / 25.14 \\
Context-gated mean fusion &82.03 / 46.89&73.18 / 40.06&69.94 / 38.20& 62.13 / 31.20\\
\hline
\end{tabular}
\end{center}
\caption{Binary / Seven-class classification results (\%) of naiive fusion models and the proposed context-gating under end-to-end white-box attack on MOSI}
\end{table*}



\begin{table*}[t]
\centering
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Model & \multicolumn{3}{c|}{Perturbed Vision} & Model & \multicolumn{3}{c|}{Perturbed Motion} & Model & \multicolumn{3}{c|}{Perturbed Audio} \\ \hline
%
 & Clean & Adv & Adv-F & & Clean & Adv & Adv-F & & Clean & Adv & Adv-F \\ \hline
%
Vision (LB) & 18.7 (54.2) & 0.0 (0.8) & 0.0 (0.0) &  Motion (LB) & 19.0 (48.4) & 0.0 (0.5) & 0.0 (0.0) &   Audio (LB) & 12.1 (35.9) & 0.0 (0.1) & 0.0 (0.0) \\ \hline
%
Concat Fusion & 30.2 (60.8) & 0.1 (8.9) & 0.0 (2.8) &   Concat Fusion & 30.2 (60.8) & 0.1 (7.5) & 0.0 (1.8) &   Concat Fusion & 30.2 (60.8) & 0.2 (8.1) & 0.0 (1.5) \\ \hline
%
Mean Fusion & 27.9 (59.7) & 0.0 (20.2) & 0.0 (8.8) &   Mean Fusion & 27.9 (59.7) & 0.0 (10.7) & 0.0 (10.7) &   Mean Fusion & 27.9 (59.7) & 0.0 (4.6) & 0.0 (4.6) \\ \hline
%
Motion+Audio (UB) & 21.9 (52.2) & 21.9 (52.2) & 21.9 (52.2) &   Vision+Audio (UB) & 23.8 (55.9) & 23.8 (55.9) & 23.8 (55.9) &   Motion+Audio (UB) & 25.6 (58.2) & 25.6 (58.2) & 25.6 (58.2) \\ \hline
\end{tabular}
\vspace{0.1cm}
\caption{Top-1 classification accuracy results on EPIC-Kitchens dataset. Higher is better. Standard multimodal fusion layers (mean, concat) are evaluated under single-source adversarial perturbations. LB = lower bound given by a unimodal model. UB = upper bound given by a multimodal model that excludes the perturbed modality.  Although there are three input modalities, perturbations (Adv, Adv-F) on a single modality are surprisingly effective, even when the adversary does not have access to the fusion layer weights (Adv-F). \karren{Full tables with results of top-5 classification accuracy, feature-level attack, noisy and mismatch corruptions are relegated to Supplementary Material but should be mentioned in the text.}}
\label{table:standard-fusion-epic-kitchens}
\end{table*}


\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{|l|c|c|l|c|c|l|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{\textbf{Clean}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Visual (RGB)\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} \\ \hline
\textbf{Baseline} &
  96.1 / 93.5 / 86.8 &
  85.7 / 81.5 / 77.0 &
  93.2 / 87.7 / 83.2 &
  15.6 / 14.3 / 14.8 &
  13.6 / 10.7 / 10.3 &
  13.8 / 12.3 / 12.9 \\ \hline
\textbf{Mean} &
  96.5 / 93.6 / 86.6 &
  84.3 / 77.7 / 73.4 &
  91.9 / 86.7 / 81.8 &
  13.2 / 12.6 / 13.1 &
  18.1 / 15.2 / 14.2 &
  11.9 / 10.5 / 10.2 \\ \hline
\textbf{Concat} &
  \multicolumn{1}{l|}{80.5 / 71.4 / 67.3} &
  \multicolumn{1}{l|}{69.0 / 64.2 / 61.3} &
  75.7 / 80.0 / 75.3 &
  \multicolumn{1}{l|}{3.71 / 3.95 / 4.62} &
  \multicolumn{1}{l|}{16.9 / 15.4 / 14.3} &
  16.4 / 13.9 / 13.2 \\ \hline
\textbf{Feature-Gated} &
  \multicolumn{1}{l|}{90.6 / 89.4 / 82.8} &
  \multicolumn{1}{l|}{81.5 / 74.7 / 72.6} &
  92.9 / 84.6 / 81.8 &
  \multicolumn{1}{l|}{67.3 / 57.2 / 53.1} &
  \multicolumn{1}{l|}{62.0 / 54.2 / 50.7} &
  68.6 / 56.0 / 53.1 \\ \hline
\textbf{Ours} &
  \multicolumn{1}{l|}{95.6 / 90.6 / 83.9} &
  \multicolumn{1}{l|}{84.5 / 79.9 / 75.7} &
  90.4 / 85.4 / 80.6 &
  \multicolumn{1}{l|}{\textbf{89.6 / 85.1 / 78.9}} &
  \multicolumn{1}{l|}{\textbf{80.5 / 73.9 / 69.8}} &
  \textbf{87.9 / 82.3 / 77.6} \\ \hline
\textbf{$\Delta$} &
   &
   &
   &
   &
   &
   \\ \hline
\end{tabular}
\caption{Average Precision results for KITTI}
\label{table:kitti-robustness-results-1}
\end{table*}


\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{|l|c|c|l|c|c|l|}
\hline
\textbf{Fusion} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Depth (Velo)\\ Perturbation\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Stereo Disparity\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} &
  \textbf{Car} &
  \textbf{Ped} &
  \multicolumn{1}{c|}{\textbf{Cyc}} \\ \hline
\textbf{Baseline} &
  3.43 / 1.58 / 1.59 &
  11.3 / 11.1 / 11.4 &
  8.72 / 8.82 / 8.22 &
  7.37 / 3.57 / 3.44 &
  8.08 / 4.64 / 4.36 &
  9.13 / 7.23 / 7.72 \\ \hline
\textbf{Mean} &
  6.77 / 3.16 / 2.90 &
  13.7 / 12.9 / 12.8 &
  10.1 / 7.88 / 8.07 &
  6.88 / 3.08 / 2.73 &
  9.17 / 8.03 / 8.81 &
  12.2 / 7.77 / 7.28 \\ \hline
\textbf{Concat} &
  \multicolumn{1}{l|}{7.30 / 6.83 / 6.73} &
  \multicolumn{1}{l|}{24.4 / 20.6 / 18.9} &
  28.8 / 24.8 / 24.7 &
  \multicolumn{1}{l|}{10.1 / 9.39 / 9.50} &
  \multicolumn{1}{l|}{26.0 / 24.2 / 21.8} &
  25.7 / 24.7 / 23.8 \\ \hline
\textbf{Feature-Gated} &
  \multicolumn{1}{l|}{51.7 / 46.5 / 43.2} &
  \multicolumn{1}{l|}{53.5 / 45.7 / 42.1} &
  58.8 / 45.6 / 53.8 &
  \multicolumn{1}{l|}{43.9 / 41.6 / 38.8} &
  \multicolumn{1}{l|}{53.9 / 47.4 / 44.1} &
  60.0 / 48.8 / 46.8 \\ \hline
\textbf{Ours} &
  \multicolumn{1}{l|}{\textbf{92.8 / 87.8 / 79.4}} &
  \multicolumn{1}{l|}{\textbf{78.3 / 71.1 / 67.1}} &
  \textbf{88.9 / 85.8 / 81.1} &
  \multicolumn{1}{l|}{\textbf{92.8 / 89.8 / 83.1}} &
  \multicolumn{1}{l|}{\textbf{83.6 / 76.8 / 72.4}} &
  \textbf{88.1 / 84.7 / 79.9} \\ \hline
\textbf{$\Delta$} &
   &
   &
   &
   &
   &
   \\ \hline
\end{tabular}
\caption{Average Precision results for KITTI}
\label{table:kitti-robustness-results-2}
\end{table*}


\begin{table}[]
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{17}{|c|}{\textbf{EPIC-Kitchens}} \\ \hline
\textbf{Odd-one-out network} &
  \multicolumn{4}{c|}{\textbf{Clean}} &
  \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Visual\\ Perturbation\end{tabular}}} &
  \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Motion\\ Perturbation\end{tabular}}} &
  \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Audio\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Detect} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} &
  \textbf{Detect} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} &
  \textbf{Detect} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} &
  \textbf{Detect} &
  \textbf{Verb} &
  \textbf{Noun} &
  \textbf{Action} \\ \hline
\textbf{Random} &
  25.0 &
  - &
  - &
  - &
  25.0 &
  - &
  - &
  - &
  25.0 &
  - &
  - &
  - &
  25.0 &
  - &
  - &
  - \\ \hline
\textbf{Unaligned features} &
  \textbf{66.8} &
  \textbf{61.5} &
  \textbf{42.5} &
  \textbf{31.4} &
  \textbf{73.4} &
  \textbf{48.0} &
  \textbf{24.2} &
  \textbf{16.8} &
  \textbf{88.6} &
  \textbf{48.5} &
  \textbf{35.6} &
  \textbf{21.1} &
  \textbf{84.7} &
  \textbf{46.5} &
  \textbf{33.3} &
  \textbf{22.1} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Aligned features\\ (Logits)\end{tabular}} &
  55.9 &
  \textbf{61.5} &
  38.0 &
  31.2 &
  54.7 &
  38.7 &
  19.5 &
  13.1 &
  41.3 &
  37.0 &
  29.1 &
  16.7 &
  52.8 &
  31.1 &
  23.9 &
  13.8 \\ \hline
\multicolumn{17}{|c|}{\textbf{KITTI}} \\ \hline
\textbf{Odd-one-out network} &
  \multicolumn{4}{c|}{\textbf{Clean}} &
  \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Visual (RGB)\\ Perturbation\end{tabular}}} &
  \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Depth (Velo)\\ Perturbation\end{tabular}}} &
  \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Stereo Disparity\\ Perturbation\end{tabular}}} \\ \hline
\textbf{} &
  \textbf{Detect} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} &
  \textbf{Detect} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} &
  \textbf{Detect} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} &
  \textbf{Detect} &
  \textbf{Car} &
  \textbf{Pedest.} &
  \textbf{Cyclist} \\ \hline
\textbf{Random} &
  25.0 &
  - &
  - &
  - &
  25.0 &
  - &
  - &
  - &
  25.0 &
  - &
  - &
  - &
  25.0 &
  - &
  - &
  - \\ \hline
\textbf{Unaligned features} &
  \textbf{96.2} &
  \textbf{90.6} &
  \textbf{79.9} &
  \textbf{85.4} &
  \textbf{93.5} &
  \textbf{85.1} &
  \textbf{73.9} &
  \textbf{82.3} &
  \textbf{98.2} &
  \textbf{87.8} &
  \textbf{71.1} &
  \textbf{85.8} &
  \textbf{98.0} &
  \textbf{89.8} &
  \textbf{76.8} &
  \textbf{84.7} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Aligned features\\ (Bounding Boxes)\end{tabular}} &
  91.9 &
  90.2 &
  76.1 &
  83.3 &
  86.8 &
  77.6 &
  66.5 &
  73.8 &
  94.4 &
  83.1 &
  64.8 &
  68.3 &
  90.4 &
  80.0 &
  65.1 &
  44.9 \\ \hline
\end{tabular}
\caption{Aligned v. unaligned features}
\end{table}

==> supp_files/task_analysis.tex <==

\begin{table}[]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
& \textbf{Verb}                    & \textbf{Noun}                    & \textbf{Action}                  \\ \hline
\textbf{Vision} & 39.6 / 83.1                      & 35.4 / 60.8                      & 18.7 / 54.2                      \\ \hline
\textbf{Motion} & 53.2 / 83.4                      & 28.6 / 53.5                      & 19.0 / 48.4                      \\ \hline
\textbf{Audio}  & 40.7 / 77.3)                      & 20.6 / 40.9                      & 12.1 / 35.9                      \\ \hline\hline
\textbf{V+M}    & \multicolumn{1}{l|}{53.9 / 85.4} & \multicolumn{1}{l|}{39.2 / 64.6} & \multicolumn{1}{l|}{25.6 / 58.2} \\ \hline
\textbf{V+A}    & \multicolumn{1}{l|}{50.0 / 84.3} & \multicolumn{1}{l|}{37.2 / 63.4} & \multicolumn{1}{l|}{23.8 / 55.9} \\ \hline
\textbf{M+A}    & \multicolumn{1}{l|}{55.8 / 84.6} & \multicolumn{1}{l|}{31.4 / 57.8} & \multicolumn{1}{l|}{21.9 / 52.2} \\ \hline \hline
\textbf{V+M+A}  & 59.0 / 86.1                      & 42.1 / 66.5                      & 30.2 / 60.8                      \\ \hline
\end{tabular}


\caption{\textbf{EPIC-Kitchens Multimodal Benchmark Task}. Top-1 / Top-5 classification accuracy of standard 1-modal, 2-modal, and 3-modal models on the Epic-Kitchens verb, noun, and action recognition task. Rows 2-4 show the performance of 1-modal models based on individual modalities; rows 5-7 show the performance of 2-modal models on every pair of modalities, and row 8 shows the performance of the 3-modal model on all of the modalities. }
\label{table:epic-kitchens-task}
\end{table}

\begin{table*}[]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
                      & \textbf{Car}                        & \textbf{Pedestrian}                 & \textbf{Cyclist}               \\ \hline
\textbf{RGB}          & 93.3 / 92.9 / 86.0                      & 82.3 / 76.3 / 71.9                      & 90.3 / 83.0 / 80.4                      \\ \hline
\textbf{Velodyne}     & 89.6 / 87.0 / 81.0                      & 82.2 / 76.2 / 72.1                      & 91.7 / 84.6 / 81.8                      \\ \hline
\textbf{Stereo Depth} & 93.9 / 88.3 / 81.6                      & 79.8 / 71.7 / 67.8                      & 83.8 / 80.4 / 75.7                      \\ \hline\hline
\textbf{R+V}          & \multicolumn{1}{l|}{93.3 / 92.8 / 86.2} & \multicolumn{1}{l|}{85.0 / 80.5 / 76.3} & \multicolumn{1}{l|}{95.1 / 87.4 / 85.1} \\ \hline
\textbf{R+S}          & \multicolumn{1}{l|}{96.1 / 93.2 / 86.5} & \multicolumn{1}{l|}{84.6 / 79.3 / 75.0} & \multicolumn{1}{l|}{90.3 / 85.3 / 82.7} \\ \hline
\textbf{V+S}          & \multicolumn{1}{l|}{93.5 / 90.4 / 83.8} & \multicolumn{1}{l|}{87.0 / 80.1 / 76.0} & \multicolumn{1}{l|}{93.4 / 86.4 / 84.0} \\ \hline \hline
\textbf{R+V+S}        & 96.1 / 93.5 / 86.8                      & 85.8 / 81.5 / 77.0                      & 93.2 / 87.7 / 83.2                      \\ \hline
\end{tabular}


\caption{\textbf{Kitti Multimodal Benchmark Task}. Average Precision of standard 1-modal, 2-modal, and 3-modal models on Easy / Medium / Hard object detection as defined by the official KITTI evaluation server \cite{KITTI_OD}. Rows 2-4 show the performance of 1-modal models based on individual modalities; rows 5-7 show the performance of 2-modal models on every pair of modalities, and row 8 shows the performance of the 3-modal model on all of the modalities.}
\label{table:kitti-detection-task}
\end{table*}

\begin{table}[]
\centering
\begin{tabular}{|l|c|c|}
\hline
                      & \textbf{Two-class}                        & \textbf{Seven class}                                  \\ \hline
\textbf{Video}          & 69.09                      & 39.32      \\ \hline
\textbf{Audio}     & 59.32                      & 33.01    \\ \hline
\textbf{Text} & 75.23                      & 46.64  \\ \hline\hline
\textbf{V+A}          & 69.82 & 40.28\\ \hline
\textbf{V+T}          & 78.64 & 49.10 \\ \hline
\textbf{A+T}          & 73.36 & 47.84  \\ \hline \hline
\textbf{V+A+T}        & 79.82                 & 49.69\\ \hline
\end{tabular}


\caption{\textbf{CMU-MOSI sentiment analysis Benchmark Task}. 2-class/7-class sentiment classification accuracy (\%) of standard 1-modal, 2-modal, and 3-modal models. Rows 2-4 show the performance of 1-modal models based on individual modalities; rows 5-7 show the performance of 2-modal models on every pair of modalities, and row 8 shows the performance of the 3-modal model on all of the modalities.}
\label{table:mosi-sentiment-task}
\end{table}




\section{Analysis of Multimodal Benchmark Tasks}

In order to leverage consistency between modalities in a multimodal task to perform robust fusion, there must be shared or redundant information between them. Here, we analyze the extent to which the modalities in EPIC-Kitchens, KITTI, and CMU-MOSI are redundant, by considering the clean performance of 1-modal (unimodal), 2-modal, and 3-modal models on the task. The results in this section help shed light on the discussion of the odd-one-out network performance in the main text. Specifically, it is easier for the odd-one-out network to detect the perturbed modality for datasets such as KITTI where there is large overlap in information between data modalities; on the other hand, odd-one-out learning is more challenging on datasets such as EPIC-Kitchens where there is a fair amount of complementary information between data modalities.

\paragraph{EPIC-Kitchens Action Recognition.} The results of our assessment of the EPIC-Kitchens multimodal benchmark are shown in Supplementary Table \ref{table:epic-kitchens-task}.  We observe a trend of diminishing returns on clean performance as we add more modalities to the model, which indicates that there is redundant information between the modalities--- notice that the drop of performance is relatively small from the 3-modal models (row 8) to any of the 2-modal models (rows 5-7), especially for the verb and noun classification tasks. However, there is also a notable amount of complementary information between the modalities. For example, the visual modality contains more information for noun classification: the 1-modal vision model outperforms the 1-modal motion and audio models in noun accuracy, and the drop from the 3-modal model to the 2-modal model excluding vision yields the largest drop in noun accuracy. Likewise, the motion modality contains more information for verb classification: the 1-modal motion model outperforms the 1-modal vision and audio models in verb accuracy, and the drop from the 3-modal model to the 2-modal model excluding motion yields the largest drop in verb accuracy. Our findings are consistent with the observations in \cite{kazakos2019epic}.

\paragraph{KITTI 2D Object Detection.} 
The results of our assessment of the KITTI multimodal benchmark are shown in Supplementary Table \ref{table:kitti-detection-task}. Here, we observe that each modality achieves high performance on the task individually. The improvement of clean performance when increasing the number of modalities from 1 (rows 2-4) to 3 (row 8) is rather minimal. This demonstrates that the information between these three modalities is highly redundant, and there is little complementary information between the modalities.

\paragraph{CMU-MOSI Sentiment Analysis.} The results of our assessment of CMU-MOSI benchmark are shown in Supplementary Table \ref{table:mosi-sentiment-task}. In this task, text is the modality that carries most information and adding video improves the performance more significantly than adding audio. Comparing row 8 which uses all three modalities and row 7 which uses video and text, as well as comparing row 4 which uses video and audio with row 1 which uses only video, one can see that there exist strong redundancy between audio and video.

